Power Grid Behavioral Patterns and Risks of Generalization in Applied Machine Learning

Recent years have seen a rich literature of data-driven approaches designed for power grid applications. However, insufficient consideration of domain knowledge can impose a high risk to the practicality of the methods. Specifically, ignoring the grid-specific spatiotemporal patterns (in load, generation, and topology, etc.) can lead to outputting infeasible, unrealizable, or completely meaningless predictions on new inputs. To address this concern, this paper investigates real-world operational data to provide insights into power grid behavioral patterns, including the time-varying topology, load, and generation, as well as the spatial differences (in peak hours, diverse styles) between individual loads and generations. Then based on these observations, we evaluate the generalization risks in some existing ML works causedby ignoring these grid-specific patterns in model design and training.

==> 020background.tex <==


\section{Background: Node-Breaker and Bus-Branch Models}\label{sec: NB vs BB}

The node-breaker (NB) model, also called the bus section/circuit breaker model, gives a complete physical description of the power grid to enable direct consideration of each grid component. Specifically, it contains bus sections (i.e., nodes) at different voltage levels, circuit breakers/switching devices, transmission lines, transformers, shunts, generators and loads, etc. The true locations of metering devices can be shown in the NB model. Fig. \ref{fig:NB model} shows an NB model of a grid sub-network in the vicinity of a substation, along with meter installations.

  \begin{figure}[h]
  \begin{subfigure}[t]{0.5\textwidth}
      \centering	\includegraphics[width=\textwidth]{figures/NB_model.png}
	\caption{Node-breaker (NB) model of a grid sub-network.}
	\label{fig:NB model}
  \end{subfigure}
  \hfill
    \begin{subfigure}[t]{0.4\textwidth}
      \centering
      \includegraphics[width=\textwidth]{figures/BB_model.png}
	\caption{Bus-branch (BB) model: substation buses are merged.}
	\label{fig:BB model}
    \end{subfigure}
    \caption{Node-breaker (NB) vs. bus-branch (BB) models}
    \label{fig:NB vs BB}
  \end{figure}


The bus-branch (BB) model is a simplified representation obtained from the NB model via the network topology processor. A BB model removes the switching devices and typically represents each substation with a single bus or a few split buses at each nominal voltage level. 
%The injection buses (i.e., buses with generation, load and shunts) and zero-injection 
The buses are interconnected by branches including transmission lines, transformers, etc. 
Meanwhile, the locations (and sometimes values) of
metering devices are reassigned to reflect measurements on the BB model.
Fig. \ref{fig:BB model} shows the BB model with reassigned metering devices.

Today, most real-time analysis, optimization control, and offline planning studies use bus-branch models to represent power system networks. The lack of breaker information has several drawbacks.  Without the knowledge of substation breaker configuration and its operation during a contingency, the fault on switching devices cannot be localized precisely. Also, any data error in switch statuses presents an opportunity for a topology error to occur on the BB model. The wrong topology remains undetectable and can cause inaccurate results in real-time operations. 








